Synthesize-It-Classifier: Learning a Generative Classifier through RecurrentSelf-analysis

In this work, we show the generative capability of an image classifier network by synthesizing high-resolution, photo-realistic, and diverse images at scale. The overall methodology, called Synthesize-It-Classifier (STIC), does not require an explicit generator network to estimate the density of the data distribution and sample images from that, but instead uses the classifier's knowledge of the boundary to perform gradient ascent w.r.t. class logits and then synthesizes images using Gram Matrix Metropolis Adjusted Langevin Algorithm (GRMALA) by drawing on a blank canvas. During training, the classifier iteratively uses these synthesized images as fake samples and re-estimates the class boundary in a recurrent fashion to improve both the classification accuracy and quality of synthetic images. The STIC shows the mixing of the hard fake samples (i.e. those synthesized by the one hot class conditioning), and the soft fake samples (which are synthesized as a convex combination of classes, i.e. a mixup of classes) improves class interpolation. We demonstrate an Attentive-STIC network that shows an iterative drawing of synthesized images on the ImageNet dataset that has thousands of classes. In addition, we introduce the synthesis using a class conditional score classifier (Score-STIC) instead of a normal image classifier and show improved results on several real-world datasets, i.e. ImageNet, LSUN, and CIFAR 10.

==> extra.tex <==
% Suppose that our dataset consists of i.i.d. samples $\{\textbf{x}_{i}\in \mathcal{R}^{D}\}_{i=1}^{N}$ from an unknown distribution $p_{data}(\textbf{x})$. We use Metropolis-adjusted Langevin algorithm (\textit{MALA}) that approximates a given distribution $p(f)$, described as \textit{MALA}-approx in \cite{nguyen2017plug}. 
\begin{equation}
    f_{t+1} = f_{t} + \epsilon_{12}\nabla \log p(f_{t}|y=y_{c}) + \mathcal{N}(0, \epsilon_{3}^{2})
\end{equation}

\subsection{Activation Maximization}
Assume we wish to sample from a conditional model $p(f|y)$,
which is proportional to a “product of experts” [19] in which each expert determines whether a soft
constraint is satisfied. First, a $p(y|f)$ expert determines a
condition for features of a an image. Also, in a high-dimensional image
space, a good $p(f)$ expert is needed to ensure the search
stays in the manifold of image distribution that we try to
model (e.g. images of faces [6, 63], shoes [67] or natural images [37]), otherwise we might encounter “fooling” examples that are unrecognizable but have high $p(y|f)$
[38, 51]. Thus, $p(f)$ and $p(y|f)$ together impose a complicated high-dimensional constraint on image generation. into an image model and a classification model:
\begin{equation}
    p(f|y) \propto p(f) p(y|f)
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Learning the Model:}
\subsection{Description of Components:}
\paragraph{Encoder $E_{\phi}(.)$:} The encoder has the following modules: (i) $READ(.)$ that receives as input the ground truth image $\textbf{x}$, decides to focus on a part of $\textbf{x}$ using an attention mechanism, and outputs vector $\textbf{r}_{t}$ (which is rasterized from the patch being attended to); (ii) an LSTM network $ERNN(.)$ that receives $(\textbf{r}_{t}, y)$, the latent representation $\textbf{h}^{enc}_{t-1}$ from a previous time step, and provides a feature vector $r_{t}$; and (iii) a write module $W(.)$ that iteratively updates a cumulative canvas matrix $\textbf{c}_{t}$. The working principle of the encoder network is summarized as follows:
\begin{equation}
\label{eq_draw}
\begin{split}
    &\widetilde{\textbf{x}}_{t} = \textbf{x} -  \zeta(\textbf{c}_{t-1}),\\
    & \textbf{r}_{t} = READ(\textbf{x},\widetilde{\textbf{x}}_{t}, \textbf{r}_{t-1})\\
    & [\textbf{s}_{t}, h^{enc}_{t}] = ERNN(\textbf{r}_{t}, h^{enc}_{t-1});\\
    &\textbf{c}_{t} = \textbf{c}_{t-1} + W(h^{enc}_{t})
\end{split}
\end{equation}
The implementation of the read and write modules are similar to the attention mechanism in \cite{gregor2015draw}, although we use it differently.
\paragraph{Classifier $C_{\theta}(.)$:}
\begin{equation}
    \begin{split}
        \mathcal{L}_{cls} = - \log C(y_{c}|f_{T})
    \end{split}
\end{equation}

==> nothing.tex <==
1.
2.
3. Methodology
    
4.

==> sections/8_rebuttal.tex <==
\noindent\textbf{Recap}: Recurrent self-analytic classifier \stic trained mixup VRM. Novel Gram-matrix Reg. MALA (\textbf{GRMALA}) for image synthesis. Attentive-\stic (\textbf{A-\stic}), Score-\stic (\textbf{S-\stic}) for GRMALA fast mixup.\\
\noindent Thank you that \textbf{\ra, \rb, \rc} found \stic interesting, significant improvement w.r.t. SOTAs (\rb, \rc), img. gen. w/o a separate generator (\rc, \ra), proposed GRMALA novel contribution (\ra, \rb, \rc). (\textit{Abbrv.}; \textbf{w/t}: with, \textbf{w/o}: without)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%
%%%
%
\vspace{-0.9cm}

\Pointilles{1}
\vspace{-0.4cm}

\noindent$@$\textbf{\rb}, $@$\textbf{\ra}, \textbf{GRMALA steps, langevin steps}: GRAMALA iteration chains at train and test; \stic: 100, A-\stic: 30, S-\stic: 70 (\textit{vs}. MCMC 200 itr. in PnP \cite{nguyen2017plug}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%
%%%
%
\vspace{-0.5cm}

\Pointilles{1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%
%%%
%
\vspace{-0.4cm}

\noindent $@$\textbf{\ra, clarification about generated. imgs, Cls$_{R/G}$ metrics calculated in Table 1:} Thank you for pointing it out! \stic-generated imgs. are used at testing/evaluation of the classifier (L615, \textbf{Cls}$_{R}$). \stic-generated imgs are used to train a classifier and validated with real imgs (L618, \textbf{Cls}$_{G}$), as proposed in [\textcolor{green}{I}]. Training time vs. loss is shown in Fig \textcolor{red}{6} ($\grave{a}$ la training w/o generation: \ra), thus showing improvement. We tried to show through \textbf{Cls}$_{G}$ that, training classifiers \textit{purely} using generated images of INN, WINN, PnP, JEM, EBM, BigGAN and SNGAN reduces the classification accuracy of ResNt/ WResNet/MobNet/GLt on CIFAR10, ImageNet and LSUN dataset (similar to [\textcolor{green}{I}]). But, \stic has shown an improved result (Tbl \textcolor{red}{1}, \textbf{Cls}$_{G}$ col.). For example: ResNt/ WResNet/MobNet/GLt trained with BigGAN gen. imgs. and tested on real images show classification acc. 43/40/39/31 on \textbf{ImageNet} [\textcolor{green}{I}], see \textbf{below Table} \underline{kindly zoom}, w.r.t \stic: 63/63/83/80 (Tbl. \textcolor{red}{1} last column);
%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.4cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%
%%%%
%
\begin{table}[h]
\centering
\resizebox{0.3\textwidth}{!}{
\begin{tabular}{llllllll}
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{INN} &
  \multicolumn{1}{c}{WINN} &
  \multicolumn{1}{c}{PnP} &
  \multicolumn{1}{c}{JEM} &
  \multicolumn{1}{c}{EBM} &
  \multicolumn{1}{c}{BigGAN} &
  \multicolumn{1}{c}{SNGAN} \\ \toprule
LSUN &
  \begin{tabular}[c]{@{}l@{}}20/29\\ /10/18\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}23/31\\ /38/19\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}62/70\\ /80/73\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}60/70\\ /80/72\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}22/22\\ /19/17\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}41/40\\ /38/35\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}55/50\\ /51/38\end{tabular} \\ \midrule
CIFAR10 &
  \begin{tabular}[c]{@{}l@{}}10/08\\ /14/07\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}19/10\\ /05/09\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}50/46\\ /49/50\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}55/50\\ /49/49\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}16/19\\ /10/09\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}52/50\\ /53/51\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}58/60\\ /59/59\end{tabular} \\ \midrule
ImageNet &
  \begin{tabular}[c]{@{}l@{}}05/02\\ /03/04\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}07/03\\ /02/03\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}38/30\\ /36/30\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}41/30\\ /37/30\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}20/18\\ /10/19\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}43/40\\ /39/31\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}43/39\\ /31/30\end{tabular} \\ \hline
\end{tabular} 
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%
%%%
%
\vspace{-0.4cm}

\noindent We missed to report this observation and we thank \ra for pointing that out. We note a similar cls. acc. improvement for \textbf{Cls}$_{R}$. We will add a description of this in final version.\\
\noindent $@$\textbf{\ra, \stic is faster than BigGAN, SNGAN?} Yes, primarily due to instability of GANs (see L693). \stic uses feedforward-feedback of a classifier and doesn't involve: adversarial game, lengthy MCMC or variational inference. Discussion on run time cmp. for LSUN (128$\times$128), CIFAR (32$\times$32), ImageNet (512$\times$512), see. L691. For ImageNet, 128$^{2}$ or lesser resolutn. (for SNGAN) \stic is $\sim 5\times$ fast.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%%%%%%%
%%%
%
\vspace{-0.5cm}

\Pointilles{1}
\vspace{-0.4cm}

\noindent $@$\textbf{\rb, Cls. as gen. is not novel:} We partially disagree; Ref \cite{gatys2016image} studied content and style transfer of images and not a generative model. Recurrent elimination of the class regions \& Gram-matrix reg. MALA sampler (that captures style ) to search using mixup VRM, A-\stic, S-\stic are not studied in any of the SOTAs \cite{gatys2016image, nguyen2017plug,jin2017introspective, grathwohl2019your}.\\
\noindent $@$\textbf{\rb, Run time complexity?} Yes. L690-L698 provide run time comp: \stic is $\sim 3.2\times$ faster than BigGAN, SNGAN. The PnP, INN, WINN have $>$ 2 nets, slower than \stic. We'll add detailed runtime analysis to the final version.\\
\noindent $@$\textbf{\rb, Comp. w/t GANs}: Considering the focus on synthesis from a classifier \& sampling using GRMALA, we show comp. with such line of works: INN, WINN, EBM, JEM and PnP. Quantitative comp. w/t two SOTA GAN methods, \textit{viz.} SNGAN \& BigGAN, are provided in Tbl. \textcolor{red}{1}.\\
\noindent  $@$\textbf{\rb,  Precision and Recall, $k$ nearest:}
\vspace{-0.35cm}

\begin{figure}[h]
  \centering
  \includegraphics[height=0.12\textwidth,width=0.33\textwidth]{images/P_R_K.png}
  \label{fig_P_R_K}
  \vspace{-0.45cm}
  
\end{figure}
\noindent \underline{Pl. zoom}, Fig (A), different initializtns of methods. High precision, recall for \stic justifying our claims in Sec \ref{sec_experiments_and_results}. Fig (B) shows precision and recall at different $k$-NN using features of ResNet-50. We'll add this info. in the final ver.

\\
%%%%%%%%%%%%%%%%%%%
%%%%%%%
%%
%
\vspace{-0.5cm}

\Pointilles{1}
\vspace{-0.3cm}

\noindent $@$\textbf{\rc, the setup works w/o $p(x)$ term}: Excellent question and sorry for the inconvenience! Softmax of the classifier $p_{\theta}^{\tau+1}(y|x)$ is, $\frac{\exp(p_{\theta}^{\tau + 1}(x)[y])}{\sum_{y^{'}}\exp(p_{\theta}^{\tau+1}(x)[y^{'}])}$ (Eqn \textcolor{red}{4}). We can \textit{approx.} $p(x,y)$, i.e. $p_{\theta}^{\tau+1}(x,y) = \exp(p_{\theta}^{\tau}(x)[y])/Z(\theta)$, we get $p_{\theta}^{\tau}(\cdot)$ from prev. time step $\tau$. Marginalizing $y$ from $p_{\theta}^{\tau+1}(x,y)$, i.e. $p_{\theta}^{\tau+1}(x)=\sum_{y} p_{\theta}^{\tau+1}(x,y)= \sum_{y} \exp(p_{\theta}^{\tau}(x)[y])/Z(\theta)$ provides us the estimation of $p(x)$, described in Eqn \textcolor{red}{5}, Alg \textcolor{red}{1} and L444. However, $p(x)$ is dropped from Eqn \textcolor{red}{1} as there is no explicit network and the learning is incorporated through GRMALA & $p_{\theta}^{\tau}(\cdot)$.\\
\noindent $@$\textbf{\rc, PnP vs. \stic}: PnP has a separate $p(x)$ network for marginal and that for \stic is the $p_{\theta}^{\tau}(\cdot)$ (see L444-L449). \underline{Advantage}: use prev. time step instead of separate $p(x)$ net.\\
\noindent\textbf{$@$\rc, Rec. self-estm., do we use actual recurrent net?} No. L445-L449 describe that a single classifier re-estimates class boundaries after each pass $\tau$ and it is trained for $50k$ iterations ($\tau\in \{1, 2, \cdots, 10\}$, L518). We sample at different itr. and show results in Fig \textcolor{red}{3}.b. \\
\noindent\textbf{$@$\rc, Theoretical work}: Thanks for sharing this thought! In addition to theoretical justification in L1228-L1325 and including the above $p(x)$ justification in the paper, studying \stic theoretically will be an important future work.\\
\noindent\textbf{$@$\rc, Ablation Mixup}:(i) \underline{MIS} scores of \stic trained with ERM \textit{vs.} \stic trained with Mixup VRM: 30/\textbf{93.61}, 20/\textbf{97.91}, 27.19/\textbf{98.62}; (ii)\underline{FID}: 35.92/\textbf{13.32}, 48.17/\textbf{12.81}, 38.27/\textbf{15.01}; on LSUN, CIFAR, ImageNet. We also note \stic-w/o VRM and recurrent self analysis, \underline{MIS}: 10, 14, 10; FID: 79, 97.01, 77.81; showing the efficacy of \stic.\\
\noindent\textbf{$@$\rc, Ablation Gram Mat.}: We use the style rep. of deeper layers, `conv21'-`conv28', and got FID: 15.01 on ImageNet. We note shallow layers `conv1'-`conv20' gives FID: 28; doesn't capture more style. Considering all layers `conv1'-`conv28' FID:30, mixes learning of deeper style and shallow layer style, thus leading to bad FID.\\
\noindent\textbf{$@$\rc, Decoder in Attentive-\stic}: L1131 in Suppl. Mat.
%%%%%%%%%%%%
%%%%%%
%
\vspace{-0.5cm}

\Pointilles{1}
\vspace{-0.4cm}
\noindent\textbf{(Reference)}: {\footnotesize
\noindent\textcolor{green}{I.} Ravuri, Seeing is not Believing, ICLR 2019
}
